C-Code Reader of Form Factors

The process $\Lambda_b \rightarrow \Lambda_c \ell^- \bar{\nu}_\ell$ serves as a tool for exploring new physics, with contributions from scalar, vector, and tensor hadronic currents in various models. These form factors are derived from the quark model or lattice QCD. This work introduces a C-code for efficiently reading lattice QCD form factors for these currents, significantly outperforming a previous Mathematica-based approach, with a speed improvement of over 64 times per data point. The code, available on GitHub $(https://github.com/darkfiresmith96/Lattice_QCD)$, also features a web interface for user inputs.

==> gui.tex <==
\section{Web Application with Graphical Interface}

If we just distribute our C source code to our users, the users will be
responsible for compiling the C source code and run them on the Linux
command-line on a computer with reasonable performance. To make our C program
available to a boarder spectrum of users, we built a prototype web
application\footnote{\url{https://qcd.herokuapp.com/}. We can provide the
source code if requested. Since we used a free instance for our prototype, the
server may go to sleep if there is no active connection for a while. When the
server is asleep, there is longer response time as the server needs to wake up.
Once it's awake, the connection shall be fast.}. The application was built
using the Node.js framework. A user can upload required data documents and
input the related parameters, see the interface in~Fig.\ref{fig:web-interface}.
The web application will then pass the inputs to the C program and run the
program on the same server.  The raw data computed will be delivered to the
user on the webpage. The prototype system is built on the Heroku Cloud
Application\footnote{\url{https://www.heroku.com/}} using a ``free-tier
instance''.  By using a cloud platform and a Docker build, we can switch to
more powerful computational resources quickly and seamlessly.

\begin{figure}[h]
 \centering
 \includegraphics[width=0.8\textwidth]{web-interface.png}
 \caption{Web interface for user inputs}
 \label{fig:web-interface}
\end{figure}

As part of the future work, we generalized this interface to allow the user to
input a mathematical expression. The user will then upload matching data files,
as depicted in
Fig.~\ref{fig:web-future}\footnote{\url{https://qcd.herokuapp.com/test}}. Our
prototype application will parse the formula text in Latex format and generate
code to compute the result of the expression from the inputs in the uploaded
data files. For example, if a user inputs an expression $\frac{1}{x} + y$ as
depicted in Fig.~\ref{fig:web-future}, and the input file can be a spreadsheet
whose column names are ``x'' and ``y'' and each column contains a list of
values. The application will compute the list of results according to the
expression. As of now, the prototype application generates Javascript code to
compute the results. In the future, C code will be generated and compiled to
ensure the efficiency.

\begin{figure}[h]
 \centering
 \includegraphics[width=0.8\textwidth]{web-future.png}
 \caption{Web application which can parse user's expression}
 \label{fig:web-future}
\end{figure}

